Efficient PAC Learnability of Dynamical Systems Over Multilayer Networks

Networked dynamical systems are widely used as formal models of real-world cascading phenomena, such as the spread of diseases and information. Prior research has addressed the problem of learning the behavior of an unknown dynamical system when the underlying network has a single layer. In this work, we study the learnability of dynamical systems over multilayer networks, which are more realistic and challenging. First, we present an efficient PAC learning algorithm with provable guarantees to show that the learner only requires a small number of training examples to infer an unknown system. We further provide a tight analysis of the Natarajan dimension which measures the model complexity. Asymptotically, our bound on the Nararajan dimension is tight for almost all multilayer graphs. The techniques and insights from our work provide the theoretical foundations for future investigations of learning problems for multilayer dynamical systems.

==> tex/titlepage.tex <==
% !TEX root = ./main.tex

\begin{titlepage}

{

%\center{\textcolor{red}{For Evaluation By PKDD Only --- Not for Public Use/Consumption\\
%To be Released at a Later Date}}

\normalsize
\rightline{\bf NDSSL Technical Report 2017-1035}
%\medskip
\vspace{0.2in}
\normalsize{\hfill{Sept. 17, 2017}}

\vspace{0.05in}
\noindent\begin{tabular}{r|p{0.75\textwidth}}
\rule[0.25in]{0pt}{0pt} & \\
Title:&\normalsize{Learning and Inference in Networked Social Systems -- Part 2:} \\
      &\normalsize{Deterministic Query Generation Methods} \\
\rule[0.5in]{0pt}{0pt} & \\
Authors: &
\small{
Abhijin Adiga\newline
Christopher J. Kuhlman\newline
Madhav V. Marathe\newline
S. S. Ravi\newline
Daniel J. Rosenkrantz\newline
Richard E. Stearns}\\

%\institute{
%Virginia Bioinformatics Institute, Virginia Tech, Blacksburg, 
%VA 24061, USA.
%Email:~ \texttt{\{ckuhlman,akumar,mmarathe\}@vbi.vt.edu} \\ \and
%Computer Science Department, University at Albany -- SUNY, 
%Albany, NY 12222, USA.
%Email:~ \texttt{\{ravi,djr\}@cs.albany.edu}
%}

\rule[0.25in]{0pt}{0pt} & \\
Contact: &
\small{Madhav V. Marathe\newline
 Email: {\tt mmarathe@bi.vt.edu} \newline
 Tel.: +1 540 231 8832\newline
 Fax: +1 540 231 2891} \\
\rule[0.25in]{0pt}{0pt} & \\

%To Appear In: &
%%Submitted To: &
%\small{The 10th IEEE International Conference on e-Science (eScience 2014)}\\
%%\small{}\\


\rule[0.25in]{0pt}{0pt} & \\
Acknowledgments: & \small{
We convey our special thanks to 
Noshir Contractor (Northwestern University),
Joshua Epstein (New York University),
Brian Goode (Virginia Tech),
Michael Macy (Cornell University), 
Naren Ramakrishnan (Virginia Tech) and
Nathan Self (Virginia Tech)
for discussions on topics related to the paper.
This work has been partially supported by
DARPA Cooperative Agreement D17AC00003 (NGS2),
DTRA CNIMS (Contract HDTRA1-11-D-0016-0001),
NSF DIBBS Grant ACI-1443054 and
NSF BIG DATA Grant IIS-1633028.
The U.S. Government is authorized to reproduce and
distribute reprints for Governmental purposes notwithstanding
any copyright annotation thereon.

\bigskip

\noindent
\textbf{Disclaimer:}~ The views and conclusions contained herein are those 
of the authors and should
not be interpreted as necessarily representing the 
official policies or endorsements, either expressed
or implied, of DARPA or the U.S. Government.
} \\
\rule[0.25in]{0pt}{0pt} & \\
\end{tabular}

\vfill

\rightline{\makebox[3.5in][l]{\vbox{\small
\noindent Network Dynamics and Simulation Science Laboratory\\
Biocomplexity Institute of Virginia Tech\\
Virginia Polytechnic Institute and State University\\
%%and\\
%%Computer Science Department, University at Albany -- SUNY
}}}

%\noindent\includegraphics[width=\textwidth]{VBI_VT_Logo.eps}
\title{}
\author{}
\date{}

%\textcolor{red}{For Evaluation By PKDD Only --- Not for Public Use/Consumption}

}

\bigskip\bigskip

\begin{center}
\fbox{\fbox{\Large{\textbf{Preliminary Version:~ Please Do Not Distribute}}}}
\end{center}

\thispagestyle{empty}

\end{titlepage}

